Mass-loss Rates of 74 Bow Shock OB Stars: No Evidence for Bi-stability Behavior

Accurate measurements of wind-driven mass-loss rates are essential for understanding the evolution and fate of massive stars. Established techniques for measuring $\dot{M}$ suffer from large dispersions and become insensitive in the regime of weak-winded late-O to early B stars. We employ a promising new technique to measure stellar mass loss for \numstars~early type stars that produce infrared stellar bow shock nebulae. We use updated stellar parameters, improved parallactic distances and proper motions, and modern dust models to characterize the bow shock nebulae and obtain new measurements of mass-loss rates. $\mdot$ ranges from $2\times10^{-9}~\moperyear$ for weak-winded late-O and early B stars at $\log\left(\lstar/L_\odot\right)\approx4.5$ to $4\times10^{-6}~\moperyear$ for the most luminous stars in our sample at $\log\left(\lstar/L_\odot\right)\approx6.3$. Stellar space velocities relative to their local standard of rest are insufficient to accurately reflect the relative star-ISM velocities for the majority of our sample, which have speeds much less than canonical runaway thresholds, suggesting the pervasive influence of bulk interstellar flows in forming bow shock nebulae. Adopting a minimum relative velocity of $20~\kms$ is physically motivated and yields mass-loss rates in excellent agreement with the latest theoretical prescriptions while requiring no adjustable parameters. We find no enhancements in $\mdot$ for stars cooler than 25~kK, in agreement with modern mass-loss recipes that do not include bi-stability effects.

==> sections/introduction.tex <==

The evolution of massive stars, with masses ranging from $8\lesssim M/\msun\lesssim120$, plays a key role in many disparate areas of astrophysics including cosmology, nucleosynthesis, star formation rates, compact object production, and gravitational-wave progenitors. The birth of metal-free, very massive stars (Pop III stars) gave rise to an ionized universe rich in high-energy UV photons, known as the epoch of reionization \citep{Venkatesan2003, MadauDickinson2014, Harikane2023}. Pop III stars are thought to have played a role in the formation of supermassive black holes, a defining feature for most galaxies \citep{Volonteri2010, Inayoshi2020}. These early stars had masses exceeding 100 solar masses, and their violent deaths either by core-collapse or pair-instability supernovae, left a nucleosynthetic mark on the universe \citep{HegerandWoosley2002H, Cayrel2004}. Enrichment from massive stars then alters the initial mass function for their host galaxies and the universe as a whole, with increasing formation of low-mass stars with increasing metallicity \citep{Chon2021}. Because of the unique roles massive stars play as the predominant source of UV photons, UV fluxes in galaxies are the most observable indicator of star formation \citep{Kennicutt1998, Salim2007}. In the final stages of their evolution, before they explode as supernovae, massive stars become Wolf-Rayet (WR) or Luminous Blue Variable \citep[LBV,][]{HubbleSandage1953} stars. Stellar feedback in the forms of stellar winds, UV radiation \citep{Whitworth1979, Kim2018}, and blast waves from supernovae all perturb their immediate and large-scale environments and affect star formation rates. Massive stars produce black holes (BH) and neutron stars (NS) at the end of the main sequence. Massive star multiple systems are also the progenitors of binary BH-BH, BH-NS, and NS-NS pairs, which eventually in-spiral and produce gravitational waves when they merge \citep{Fryer2002, Pretorius2005, Kalogera2004, Abbott2016, Abbott2017a, Abbott2017b}. The exact rates of production of compact object formation are determined by the final stellar mass. To understand black holes, neutron stars, and degenerate systems, it is imperative to understand a star's evolution for both the main- and post-main-sequence phases.

%Some binary stars evolve in such a way that they orbit inside a common envelope---a process known as common envelope evolution \citep[CEE, ][]{Taam2000, Ivanova2013}. Decide if neededXX.

%Multiple physical effects shape the mass-loss rates of massive stars \citep{Puls2008, Vink2022}. In close binaries, mass transfer between components occurs when the radius of the primary star exceeds the Roche lobe---Roche Lobe Overflow (RLOF)---resulting the outer-layers of the more-evolved, more-massive primary star to the less-massive secondary. The recipient star can strip the hydrogen envelope of the donor star, known as envelope stripping. Such systems are likely the progenitors to Type Ib and Ic supernovae \citep{FryerandHeger2000, Fryer2012, Tauris2015}. Significant mass is transferred between the primary and secondary stars, with some mass leaving the system entirely, altering the production of neutron stars and black holes compared to single star evolution \citep{Sana2012, Smith2014}. These effects are especially important to consider for a holistic prescription of mass loss for massive stars, considering that the majority of massive star systems are at least binary systems \citep{KobulnickyandFryer2007, Sana2011, Moe2017}. The WR or LBV, whether originating from binary influences or single star evolution \citep{KenyonandGallagher1985, Smith2015}, can also shed a lot of mass. LBV stars can lose on the order of $~\sim1~\msun$ in just one pulsation \citep{Humphreys1994}. Averaged over time, LBV stars exhibit mass-loss rates on the order of $10^{-7}$--$10^{-5}$ $\moperyear$ \citep{Sanyal2015, Smith2017, Jiang2018}. WR stars exhibit similar mass-loss rates \citep{Crowther2007, Merritt2025}. Nevertheless, single star radiation-driven stellar winds, prior to any binary interaction, is the first mechanism for mass loss operating in all stars regardless of binarity.

Massive stars exhibit several channels through which their mass is altered throughout their lives. In binary systems, significant mass is transferred between stars when the primary overfills the Roche-lobe of the system

% Stellar winds are a dominant mechanism whcih reduces the stellar mass. LBV pulsations many solar masses at once. Binary interactions. Fryer. Heger. stripping envelopes. E name. May not be dominant mech, but its the inital phenomenon channel by which massive stars eject material through MS and post MS lifetimes. come back to winds. primary means of mass loss.

%Massive stars, typically defined as stars with masses ranging from 5--120~\msun, are the sources of some of the most brilliant phenomena in the universe. Their dominant light output outshines their more numerous, and significantly dimmer, low-mass counterparts in spiral galaxiesXXcitation. The cataclysmic death of massive stars, marked by a core-collapse supernova explosion, gives rise to the peculiar degenerate objects neutron stars and black holes, while the supernova explosion briefly rivals the luminosity of the host galaxy itself.XXcitation Since massive stars spend their tumultuous lifetimes fusing hydrogen into heavier elements, and the violent nature of their deaths, massive stars are markedly the sites of chemical enrichment in the universeXX citation.

%Hot, massive stars ($\gtrsim8$ \msun) are the sources of unique phenomena. Although fewer in number than their low-mass counterparts \citep{Massey1995, Kroupa2003}, their imprint on their host galaxy is significant. The remarkably high temperatures of massive stars make them the predominant sources of ionizing radiation in the universe. The radiation pressure from high-energy UV photons can heat up and dissociate molecular clouds that would otherwise be sites of star formation --- a process known as stellar feedback \citep{Whitworth1979, Kim2018}\footnote{Additional stellar processes also contribute to the wider phenomenon known as ``stellar feedback.'' For a comprehensive review, see \citet{Krumholz2019}}. In addition to shaping their immediate surroundings, clusters of massive stars can give rise to galactic-scale outflows \citep{Heckman1993, Bland-Hawthorn1995}. Massive stars are the progenitor objects of black holes and neutron stars. The supernovae (SNe) explosions that mark this dramatic stage of massive star evolution can fully destroy, or otherwise disrupt, nearby gas clouds and inhibit star formation to a similar, or even greater extent, than other feedback mechanisms from main-sequence stars \citep{RogerandPittard2013, Calura2015, Geen2016}. Not only do massive stars shape their local and galactic environments, massive stars chemically enrich their host galaxies with heavier elements \citep{Matteucci1986, Timmes1995, Dwek1998}. 

%XX Radiation-driven stellar wind
%% Remove, too much detail. Maybe include in dissertation 
%Ever since it was known that photons carry momentum, many have speculated whether starlight could drive outflows of material in the upper atmospheres of stars on the main sequence \citep{Johnson1925, Milne1926, Beals1929}. This effect was thought to be especially pronounced in the case of hot, luminous stars, where their high-energy photons carried more momentum and overlapped with the wavelengths of strong metal ion transitions in the ultraviolet. \citet{Parker1958} measured the first continuous outflow from a main-sequence star in his study of the solar wind. The measured mass-loss rate of $\sim$$10^{-12}\moperyear$ indicated that the impact of solar winds on the evolution of a Sun-like star is minimal. Stellar winds gained prominence when signatures of substantial stellar outflows were detected around massive stars with the birth of UV astronomy. \citet{Morton1967} obtained far-ultraviolet spectra of three O- and B-type supergiant stars. Examining the metal-resonance lines for \ion{C}{4}, \ion{N}{5}, and \ion{Si}{4}, \citet{Morton1967} observed P-Cygni features blue-shifted by 1400$\kms$, indicating a high-velocity stellar mass ejection. Their analysis yielded mass-loss rates $\sim$10$^{-6}\moperyear$. Considering the several million years stars spend in the supergiant phase, this ejection can decrease the mass of the star by a few percent, a non-negligible amount from an evolutionary perspective in some edge cases. The escaping material is accelerated in a wind at distance ranging from close to the star to a distance of several stellar radii. This acceleration proceeds until a terminal velocity on the order of 1000--2000 km/s is achieved, resulting in a steady state \citep{Milne1926, LucyandSolomon1967}. Subsequent UV observations confirmed other OB stars showed similar mass loss phenomena \citep{Morton1967b, Carruthers1968, Morton1969, Hutchings1970}.

The ubiquity of expanding atmospheres for massive stars precipitated modeling to determine how stellar parameters shaped mass-loss rates through stellar winds. \citet{CAK1975} found that considering acceleration on more-abundant hydrogen and helium rather than metal ions alone increased mass-loss predictions significantly. They predicted a dwarf O5 star would have a mass-loss rate on the order of $10^{-6}\moperyear$, corresponding to shedding $25~\%$ of its mass while on the main sequence. Quantifying mass-loss rates as a function of temperature and evolutionary phase allows predictions of the final mass of the star and the end products. , and several prescriptions have been developed. The most-prolific of which, are the relations in \citet{Vink2001}, which parametrize mass loss as a function of stellar luminosity $\lstar$, stellar mass $\mstar$, terminal wind speed $\vterm$, stellar temperature $\teff$, and metallicity $\metallicity$. Since absorption from metal ions drives the stellar wind (in part), the ionization state of the ions is an important factor when predicting mass-loss rates. This has led to the prediction of the so-called ``bi-stability'' jump, in which mass-loss rates are expected to increase by factors of several and terminal wind velocities decrease by a factor of 2 at temperatures corresponding to the recombination of wind-driving ions. The \citet{Vink2001} theoretical calculations predict an increase in mass-loss rates over the bi-stability region at $\teff=25$~kK by 5--7. Alternative prescriptions do not predict an increase in mass-loss rate over the bi-stability region \citep{Krticka2021, Bjorklund2023}. Observational attempts to measure this effect yield mixed results. \citet{Lamers1995} found the bistability of stellar winds in their study of 117 O--F stars, with stars hotter than $\teff>21$~kK showing terminal wind speed to escape velocity ratios of 2.6 and cooler stars exhibiting terminal wind speed to escape velocity ratios of 1.3. From this, \citet{Lamers1995} predicted an increase in $\mdot$~by a factor of 2 when crossing to the cool side of the bistability jump, noting the limitations of standard mass-loss techniques for less luminous stars. \citet{K19} found enhanced mass-loss rates over the bi-stability jump in their analysis of 67 OB stars. They found that stars $\teff<25$~kK show mass-loss rates several orders of magnitude larger than the \citet{Vink2001} prescription. On the other hand, \citet{Markova2008} found only modest or no increase in $\mdot$ in their small study of early to late B supergiants. \citet{deBurgos2024}, and \citet{Alkousa2025} find no increase in mass-loss rates in their studies of 116 blue- and 16 late-O and B-supergiant stars, respectively. Given the diversity of mass-loss predictions and behaviors in different regimes, measuring the mass-loss rates of large samples of massive stars is needed to constrain competing models.

%Considering radiative acceleration on particles in the outer layer of stars, \citet{Milne1926} and \citet{Beals1929} were the first to proposgfxge a scenario in which the outward radiative acceleration could exceed the inward gravitational acceleration. As the atoms accelerate away from the star, the starlight is blue(red?)-shifted, increasing the acceleration of the atoms. This is a self-sustaining effect; if the frequency exceeds the absorption frequency of the atoms, then the material decelerates until the absorbed starlight is red-shifted, and the particles accelerate again. This results in expelled layers of the star moving at constant velocity --- the terminal velocity of the wind. \citet{CAK1975} expanded upon the idea set forth by \citet{Milne1926} and \citet{Beals1929}. quantitatively predict the mass-loss rates for . Stellar winds are the dominant mechanism through which stellar mass is reduced. 

%One particular process unique to massive stars is radiation-driven stellar winds. First conceptualized by \citet{Milne1926} and \citet{Beals1929}, the high-energy photons characteristic of massive stars were long thought to impart their momentum on particles on the outer layers of the stars, creating expanding atmospheres. In addition, stellar winds are enhanced by metal-line blanketing in which . Only with the advent of UV astronomy in the works \citet{Morton1967} and \citet{LucyandSolomon1967} were these effects first observed.

%XX Methods of measuring mass loss

% New and independent techniue. Dont have to explin the filings. Reference Vink reviews. Major uncertinties micro and macro clumping eg. see review by Vink. Still need to say something mdot has been measured. Vary wildly. Known problems include clumping. Dont hve to explin ech one. phrase or two about the problem.

% DISCUSSION Several techniques for measuring mass-loss rates have been developed since the discovery of massive star stellar outflows \citep{Puls2008, Smith2014, Vink2022}. Recent works combine multiple methods to obtain consistent measurements of $\mdot$ while taking into account complicating factors \citep{Martins2005, Vink2023}. One common method makes use of the P-Cygni profiles in the UV exhibited by metal resonance transitions \citep{Garmany1981, HowarthandPrinja1989, Marcolino2009}. Two wind properties can be extracted from UV techniques, terminal wind speed $\vinfty$ and mass-loss rate $\mdot$. Terminal wind speed is the most evident of the two, as it is easily obtained from the shift in the P-Cygni profile itself. The mass-loss rate $\mdot$ requires a more rigorous analysis. With information on the abundance of a metal and its ionization fraction, the mass-loss rate can be measured from UV XXstate?C, N, and Si resonance lines. The challenge of UV techniques is that for temperatures and metallicities typical for Galactic stars, it is very common for UV metal lines to be saturated. In such cases, the derived mass-loss rate can only serve as a lower limit. The UV P-Cygni lines are analyzed using the Sobolov method, in which the optical depth of the specified line is proportional to the density of the wind $\rho$. The derived $\mdot$ too, scales with the density of the wind. As such, UV approaches are considered ``$\rho$'' diagnostics. Another technique utilizes the \halpha~recombination lines in the wind to measure mass-loss rates \citep{Leitherer1988, Lamers1993, Puls1996, Markova2004} XXprinja??. The benefit of this method is that there is no uncertainty of the ionization of hydrogen for hot stars, unlike metal species which exhibit several ionization states. As the mass-loss rate scales with $\rho^2$, and hot stars are known to exhibit small-scale density inhomogeneities---microclumping---in their winds, it is common for \halpha~methods to yield large overestimates in $\mdot$. Numerical simulations predict stellar winds to be inhomogeneous \citep{Feldmeir1997, RunacresandOwocki2002, DessartamdOwocki2005, Owocki2015}. \citet{Fullerton2006} demonstrated a large discrepancy between the $\rho$ and $\rho^2$ techniques in their comparison of \halpha~and UV mass-loss rates for 40 Galactic O stars. This discrepancy seemed to suggest microclumping was more significant than previously thought, and \halpha~methods would have to be revised significantly to account for microclumping effects. However, once thought to be independent of clumping effects, UV methods may also suffer its own complications. \citet{Oskinova2007} was the first to suggest that the treatment of clumps as optically thick, rather than optically thin, XXplaces with hight and low densitiesan effect known as ``macroclumping'' or ``porosity'', could reconcile the discrepancy found in \citet{Fullerton2006}. With this approach, \citet{Surlan2013} showed that macroclumping could help resolve this divergence. It is now understood that both \halpha~and UV methods must account for the impacts of clumping.

%Whether a star evolves into a neutron star or black hole is dependent on the star's mass at its birth and its history of mass loss \citep{Heger2003}. Although insignificant compared to mass transfer due to binary interactions, the wind-driven mass-loss rate can also sway the evolutionary course of a single star. \citet{Meynet1994} find significant evolutionary difference when simulating when ehancing wind-driven mass-loss rates by a factor of two for example. controversies.

%XX Stellar bowshock nebulae

%XX heres a different tehcnique that relies on different physics potentially no compromised by problems of other techniqes.

A new technique to measure mass-loss rates that is physically independent of existing methods uses stellar bowshock nebulae \citep{K18, K19}. XXK16SST Stellar bowshock nebulae are arc-shaped features formed when dust grains in the interstellar medium are shocked and heated by the winds of a high-velocity, early-type star. The mass-loss rate of the central star can be measured given information on the properties of the ambient interstellar medium and morphology of the resulting bowshock. \citet{GullandSofia1979} were the first to propose this technique, in their work reporting the discovery of newly discovered shocklike nebulae around a T Orionis K0e variable star, LL Ori, and an O9.5 V runaway, $\zeta$ Oph, from optical photometric data. Balancing ram pressure from the incident stellar wind on the bulk motion of the surrounding material, \citet{GullandSofia1979} found that the mass-loss rate of the central star could be calculated from

\begin{equation}
    \dot{M} = \frac{4\pi R_0^2v_*^2\rho_a}{v_w}\text{ ,}
    \label{eq:one}
\end{equation}

\noindent with $R_0$ representing the ``standoff distance'' between the star and the apex of the bowshock, $v_*$ being the velocity of the star with respect to its surroundings, $\rho_a$ signifying the ambient density of the pre-shock ISM, and $v_w$ denoting the speed of the outflowing stellar wind. Using estimates on these parameters for both bowshock nebulae, \citet{GullandSofia1979} derived independent measures of mass-loss rates for both stars. In the case of $\zeta$ Oph, their value of $2.3\times10^{-8}\moperyear$ agreed well with the contemporaneous approximation of $2.2\times10^{-8}\moperyear$, and with some contemporary measurements of $2\times10^{-8}\moperyear$ \citep{Gvaramadze2012, K19}. Using bowshock nebulae to measure mass-loss rates would remain untapped for several decades until a reformulation from \citet{K18} allowed this technique to be extended the growing collection of IR wavelength bowshock nebulae. Using the same technique developed by \citet{GullandSofia1979}, \citet{K18} refined measurements of mass-loss rates by carefully inferring interstellar number densities from archival infrared Herschel Space Observatory \citep[most targets selected from Hi-GAL survey][]{Molinari2010}XX images. \citet{K18} applied this method to measure the mass-loss rates for 20 OB stars that supported infrared bowshock nebulae. These preliminary results generally showed good agreement with some UV techniques, while showing some deviations from modern UV analysis. Comparing with \halpha-based measurements, they found their results were lower by factors of several on account of the \halpha~value weren't corrected for clumping effects. After a promising demonstration of the bowshock method, \citet{K19} expanded the bowshock sample to 70 OB stars. They found mass-loss rates ranging from $\sim10^{-7}$ to $10^{-9}\moperyear$. Interestingly, \citet{K19} found that stars on the cool side of the bistability jump (i.e. with effective temperatures $T_{\text{eff}}\lesssim 25$~kK) showed evidence for the predicted enhancement. Their analysis was based on red wavelength optical spectra, which limited the precision on determinations of effective temperature. For stars hotter than 25~kK, their results were $\sim0.4$~dex below the \citet{Vink2001} predictions showing that, on average, bowshock-derived mass-loss rates are a factor of $3$ lower than the commonly used prescription.


XX(Move to introduction)They found that bowshock stars have a similar runaway fraction (24\%) as non-bowshock O stars (22\%) selected from the Galactic O-Star Catalog \citep[][GOSC]{Maiz2013, Sota2014}. They also found that bowshock stars have a higher median space velocity (14.6$\kms$) than the control sample (11.3~$\kms$). Said another way, bowshock stars are not exclusively runaway stars, in fact most bowshock stars have space velocities less than 25~$\kms$. It's also true that not all runaway stars are not bowshock stars, in fact only (PeriXX) 10\% of runaway stars show IR bowshocks.

%Simulations paragraph, maybe useful later
%Simulations have investigated how parameters of interest impact the viability of stellar bowshock nebulae, namely the wind-driven mass loss $\mdot$, the terminal wind speed $\vinfty$, the velocity of the star with respect to its surroundings $v_*$, and the interstellar number density $n_a$ \citep{ComeronandKaper1998, Henney2019}. Simulations show that stratified layers characterized by different temperatures, densities, and pressures form around a stable stellar wind bowshock, and investigate how altering any of the parameters listed previously can cause instabilities. Simlulations also find that stellar wind bowshock nebulae are observable over a range of bandpasses, from \halpha, to the mid infrared, and including the radio \citep{Acreman2016, Meyer2016}.

%Bowshock searches, maybe include later?
%The advent of infrared all-sky space telescope surveys has revealed copious arc-like and ring-shaped structures around other stars. In their analysis of newly released Infrared Astronomical Satellite (\textit{IRAS}) data, \citet{vanBurenandMcCray1988} report 15 prominent objects discovered from 12, 60, and 100 \micron data. They classify these objects into stellar wind bubbles, stellar wind bow shocks, and radiation pressure-driven bow waves, and find 11 of the 15 prominent objects to be stellar wind bow shocks. \citet{vanBuren1995} identified 58 candidate stellar bowshock nebulae in their subsequent investigation using 60 \micron~\textit{IRAS} data. \citet{K16} performed the largest-scale search for stellar bowshock nebulae by examining 22 and 24 \micron~infrared data from Spitzer Space Telescope (\textit{SST}) and Wide Field Infrared Explorer (\textit{WISE}) survey data, and found 709 arc-shaped nebulae, with 660 of them having no previous identification. \citet{J19} added 311 candidate stellar bowshock nebulae to \citet{K16} catalog in their citizen science analysis of \textit{SST} galactic-plane survey data.

%The stellar winds of massive stars can (in some cases), sweep up the surrounding interstellar material and produce arc-shaped nebulae.
%paraphrase conclusions
%XX Overview of paper

In this work, we measure the mass-loss rates for \numstars~stars that lie at the center of bowshock nebulae in the same manner as \citet{K18, K19}, with some important improvements. The Gaia Data Release 3 \citep[\textit{Gaia} DR3,][]{GaiaDR32023} provides newer parallaxes and proper motions distances and proper motions for bowshock-driving stars. With these new data, we can expect finer precision on the  measurements, a parameter of interest when calculating mass-loss rates. In addition, \citet{Patten2025} used blue-optical spectra to obtain more precise measurements on stellar temperature $\teff$, and surface gravity $\logg$ for a large sample of bowshock-driving stars. This improvement enables more accurate estimates of terminal wind speeds $\vinfty$, another factor in mass loss rate calculations. Finally, \citet{Whisnant2025} used citizen science data to tabulate the stand-off distances $\rnaught$ for a subset of stars in the \citet{K16} and \citet{J19} bowshock catalogs, from which this work draws. These combined improvements enable more robust accurate estimates for a larger sample of early-type stars. In Section~\ref{sec:targs} we describe our target selection. In Section~\ref{sec:calculation} we review the method by which we determine the mass loss rates. In Section~\ref{sec:results} we present a table of results and compare the bowshock mass loss rates with other measurements of $\mdot$. 


%We use the results of Patten... temperatures from Patten, kinematic paramets from new gaia data. what could we cut? what does a fresh reader need to know. thin by 20 percent.

% determinations of mass-loss ratesThe result of these combined improvements is finer determinations of $\mdot$ for a larger sample of stars than those studied in \citet{K18, K19}.

% prepare discussion if its too specific for introduction. all arguments for mass loss cant go in intro. outstanding problems in mass loss, write details in discussion.

In Section~\ref{sec:targs}

==> sections/measuring_mdot.tex <==
\startlongtable
\begin{deluxetable*}{lccccccc}
	\tablecaption{Bowshock Stars}\label{tab:BSstars}
	\tabletypesize{\scriptsize}
	\tablehead{
		ID & $R_0$ & $D$ & $V_a$ & $I_\nu$ & $V_w$ & $\ell$ & $j_\nu$\\& $\farcs$ & $\kpc$ & $\kms$ & $\Jysr$ & $\kms$ & $\farcs$ & $\Jycmsrnuc$ \\
		(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)}
	\startdata
		BS001$_\star$ & 27.77 & 2.85 &19 & -inf & 2174 & 46.1 & -11.46 \\
		BS007$_\star$ & 11.13 & 1.22 &11 & 8.91 & 976 & 11.2 & -11.57 \\
		BS010$_\star$ & 3.1 & 2.46 &19 & -inf & 1538 & 41.8 & -10.75 \\
		BS013$_\star$ & 299.0 & 0.13 &17 & -inf & 1979 & 352.0 & -11.30 \\
		BS016$_\star$ & 26.54 & 3.07 &5 & 7.82 & 1496 & 20.7 & -11.14 \\
		BS019$_\star$ & 11.66 & 0.94 &26 & -inf & 1199 & -99.0 & -10.45 \\
		BS026$_\star$ & 8.6 & 3.27 &8 & -inf & 1606 & -99.0 & -99.00 \\
		BS027$_\star$ & 7.54 & 1.80 &6 & -inf & 998 & -99.0 & -11.33 \\
		BS039$_\star$ & 73.0 & 3.95 &65 & -inf & 2101 & -99.0 & -11.64 \\
		BS043$_\star$ & nan & 1.41 &8 & -inf & 1444 & -99.0 & -99.00 \\
		BS051$_\star$ & nan & 1.42 &3 & -inf & 2172 & -99.0 & -99.00 \\
		BS054$_\star$ & 95.0 & 1.46 &17 & -inf & 1541 & 128.0 & -11.71 \\
		BS056$_\star$ & 28.0 & 5.14 &21 & -inf & 1429 & -99.0 & -11.52 \\
		BS061$_\star$ & 22.44 & 2.08 &21 & -inf & 1820 & -99.0 & -11.14 \\
		BS063$_\star$ & 3.5 & 1.76 &5 & -inf & 1870 & 36.7 & -10.64 \\
		BS064$_\star$ & 24.0 & 1.72 &55 & -inf & 3443 & 36.3 & -10.95 \\
		BS065$_\star$ & 6.1 & 1.81 &3 & -inf & 862 & -99.0 & -11.23 \\
		BS066$_\star$ & 61.0 & 1.91 &23 & -inf & 2915 & 88.6 & -11.35 \\
		BS067$_\star$ & 8.47 & 1.86 &4 & -inf & 1984 & -99.0 & -10.89 \\
		BS150$_\star$ & 12.1 & 0.61 &17 & 7.88 & 1263 & 37.9 & -10.80 \\
		BS200$_\star$ & 10.13 & 4.52 &34 & -inf & 1264 & -99.0 & -10.98 \\
		BS240$_\star$ & 12.8 & 1.27 &8 & -inf & 387 & -99.0 & -11.72 \\
		BS255$_\star$ & 2.0 & 1.27 &19 & -inf & 741 & -99.0 & -10.69 \\
		BS288$_\star$ & 11.76 & 2.91 &11 & -inf & 1478 & 29.5 & -11.37 \\
		BS298$_\star$ & 21.6 & 2.70 &25 & -inf & 983 & 43.2 & -11.49 \\
		BS300$_\star$ & 6.9 & 2.05 &4 & -inf & 1675 & 32.3 & -11.03 \\
		BS302$_\star$ & 4.9 & 2.45 &62 & -inf & 940 & 24.4 & -11.09 \\
		BS303$_\star$ & 7.8 & 11.45 &52 & -inf & 763 & -99.0 & -11.13 \\
		BS305$_\star$ & 4.9 & 1.92 &39 & -inf & 2119 & 21.7 & -10.61 \\
		BS306$_\star$ & 13.67 & 2.18 &7 & -inf & 1479 & 34.7 & -11.26 \\
		BS314$_\star$ & 5.4 & 8.67 &11 & -inf & 1408 & 20.0 & -11.38 \\
		BS319$_\star$ & 21.0 & 10.50 &11 & -inf & 1117 & -99.0 & -11.78 \\
		BS320$_\star$ & 35.5 & 3.18 &7 & 7.76 & 1531 & 30.9 & -11.45 \\
		BS321$_\star$ & nan & 4.75 &1 & -inf & 1854 & -99.0 & -99.00 \\
		BS322$_\star$ & nan & 4.92 &3 & -inf & 2031 & -99.0 & -99.00 \\
		BS324$_\star$ & 25.7 & 5.32 &30 & -inf & 2001 & -99.0 & -11.56 \\
		BS325$_\star$ & 12.9 & 1.32 &-99 & -inf & 900 & -99.0 & -11.01 \\
		BS326$_\star$ & 22.7 & 3.34 &17 & -inf & 1283 & -99.0 & -11.40 \\
		BS328$_\star$ & 16.0 & 3.26 &18 & -inf & 1354 & -99.0 & -11.60 \\
		BS330$_\star$ & 25.5 & 1.71 &9 & -inf & 985 & 53.0 & -11.11 \\
		BS331$_\star$ & 25.5 & 1.69 &4 & -inf & 2243 & -99.0 & -10.96 \\
		BS332$_\star$ & 28.2 & 1.73 &5 & -inf & 1981 & 24.8 & -11.39 \\
		BS335$_\star$ & 15.6 & 2.01 &12 & -inf & 1184 & 18.8 & -11.12 \\
		BS339$_\star$ & 70.0 & 1.58 &77 & -inf & 3353 & -99.0 & -11.15 \\
		BS340$_\star$ & 15.9 & 1.47 &19 & -inf & 1337 & 37.6 & -11.12 \\
		BS341$_\star$ & nan & 1.77 &11 & -inf & 2076 & -99.0 & -99.00 \\
		BS343$_\star$ & 174.0 & 1.78 &49 & -inf & 1104 & -99.0 & -11.74 \\
		BS344$_\star$ & nan & 1.72 &45 & -inf & 3470 & -99.0 & -99.00 \\
		BS345$_\star$ & 18.5 & 0.80 &6 & -inf & 1491 & 35.8 & -11.06 \\
		BS346$_\star$ & nan & 3.68 &15 & -inf & 885 & -99.0 & -99.00 \\
		BS349$_\star$ & nan & 4.25 &20 & -inf & 1275 & -99.0 & -99.00 \\
		BS350$_\star$ & 23.0 & 2.32 &50 & -inf & 1170 & 45.1 & -11.03 \\
		BS351$_\star$ & 27.6 & 9.33 &6 & -inf & 2073 & 34.8 & -11.94 \\
		BS353$_\star$ & 30.5 & 4.64 &67 & -inf & 2545 & -99.0 & -11.50 \\
		BS354$_\star$ & nan & 7.92 &8 & -inf & 1228 & -99.0 & -99.00 \\
		BS356$_\star$ & 15.6 & 2.79 &10 & -inf & 1375 & -99.0 & -11.30 \\
		BS357$_\star$ & 21.8 & 2.74 &48 & 7.10 & 1166 & 33.6 & -11.41 \\
		BS358$_\star$ & 8.9 & 0.87 &2 & -inf & 794 & -99.0 & -11.27 \\
		BS359$_\star$ & 42.0 & 2.64 &12 & -inf & 1938 & 50.8 & -11.62 \\
		BS360$_\star$ & 35.5 & 3.03 &74 & -inf & 889 & -99.0 & -11.18 \\
		BS361$_\star$ & 91.7 & 4.56 &29 & 6.88 & 1063 & 80.4 & -12.09 \\
		BS362$_\star$ & nan & 3.89 &27 & -inf & 1256 & -99.0 & -99.00 \\
		BS364$_\star$ & nan & 2.46 &-99 & -inf & 2232 & -99.0 & -99.00 \\
		BS365$_\star$ & 29.9 & 1.06 &11 & 7.17 & 1439 & 37.0 & -11.32 \\
		BS366$_\star$ & 50.4 & 1.02 &11 & -inf & 1781 & -99.0 & -11.12 \\
		BS367$_\star$ & 36.0 & 2.10 &8 & -inf & 2013 & 40.2 & -11.45 \\
		BS368$_\star$ & 14.0 & 1.98 &8 & 8.25 & 1999 & 32.3 & -11.09 \\
		BS369$_\star$ & 94.925 & 1.96 &-99 & 7.71 & 2505 & 72.2 & -11.83 \\
		BS371$_\star$ & 51.0 & 3.00 &24 & -inf & 3219 & -99.0 & -11.64 \\
		BS372$_\star$ & 21.0 & 3.01 &16 & -inf & 1956 & -99.0 & -11.35 \\
		BS373$_\star$ & 10.0 & 0.42 &23 & -inf & 1118 & -99.0 & -10.75 \\
		BS374$_\star$ & 120.0 & 1.49 &18 & -inf & 2093 & -99.0 & -11.87 \\
		BS375$_\star$ & 9.9 & 0.39 &88 & -inf & 2083 & -99.0 & -10.47 \\
		BS376$_\star$ & 165.0 & 1.31 &21 & -inf & 3134 & -99.0 & -11.75 \\
		BS377$_\star$ & 61.0 & 6.29 &42 & -inf & 2535 & -99.0 & -12.42 \\
		BS378$_\star$ & 77.0 & 0.41 &9 & -inf & 2035 & -99.0 & -11.34 \\
		BS381$_\star$ & 71.0 & 1.38 &11 & -inf & 2769 & -99.0 & -11.29 \\
		BS383$_\star$ & 51.0 & 6.27 &88 & -inf & 2203 & -99.0 & -11.73 \\
		BS384$_\star$ & 31.0 & 3.42 &4 & -inf & 2308 & -99.0 & -11.50 \\
		BS385$_\star$ & 80.0 & 2.35 &30 & -inf & 2811 & -99.0 & -11.67 \\
		BS386$_\star$ & 53.0 & 2.02 &48 & 7.56 & 1202 & 89.7 & -11.31 \\
		BS388$_\star$ & 59.0 & 2.28 &-99 & -inf & 925 & -99.0 & -11.34 \\
		BS389$_\star$ & 11.0 & 1.81 &15 & -inf & 1185 & -99.0 & -10.96 \\
		BS634$_\star$ & 32.61 & 1.60 &9 & 7.63 & 1934 & 41.7 & -11.31 \\
		BS640$_\star$ & 6.95 & 1.56 &23 & -inf & 1486 & 20.8 & -10.81 \\
		BS662$_\star$ & 65.0 & 1.71 &13 & -inf & 2041 & 86.0 & -11.57 \\
		BS667$_\star$ & 17.0 & 1.00 &29 & 7.15 & 1724 & 28.5 & -10.92 \\
		BS673$_\star$ & 6.0 & 3.88 &21 & -inf & 1460 & -99.0 & -11.17 \\
		BS687$_\star$ & nan & 2.69 &20 & -inf & 1467 & -99.0 & -99.00 \\
		BS692$_\star$ & 34.0 & 1.79 &17 & -inf & 2449 & 52.7 & -11.27 \\
		BS700$_\star$ & 15.8 & 3.87 &16 & -inf & 1458 & -99.0 & -11.15 \\
		BS705$_\star$ & 26.9 & 2.35 &24 & -inf & 1465 & -99.0 & -11.42 \\
		BS714$_\star$ & nan & 2.70 &8 & -inf & 1146 & -99.0 & -99.00 \\
		BS715$_\star$ & nan & 1.98 &5 & -inf & 1548 & -99.0 & -99.00 \\
		BS722$_\star$ & nan & 1.82 &5 & -inf & 1045 & -99.0 & -99.00 \\
		BS778$_\star$ & 17.65 & 1.71 &-99 & -inf & 1375 & -99.0 & -10.82 \\
		BS779$_\star$ & 20.13 & 2.09 &8 & -inf & 1744 & -99.0 & -11.42 \\
		BS783$_\star$ & 19.6 & 1.43 &41 & -inf & 1770 & 39.9 & -11.27 \\
		BS792$_\star$ & 16.3 & 2.15 &4 & -inf & 2261 & 29.4 & -11.03 \\
		BS794$_\star$ & nan & 0.94 &16 & -inf & 1028 & -99.0 & -99.00 \\
		BS884$_\star$ & 13.51 & 1.85 &16 & -inf & 1424 & 29.5 & -11.15 \\
		BS885$_\star$ & nan & 0.18 &-99 & -inf & -1310 & -99.0 & -99.00 \\
		BS887$_\star$ & 56.63 & 1.79 &24 & -inf & 2736 & -99.0 & -11.31 \\
		BS892$_\star$ & 45.14 & 1.21 &10 & -inf & 2244 & -99.0 & -11.25 \\
	\enddata
	\tablecomments{(1) Stellar bowshock nebulae identifier from the K16 and addendum J19 catalogs; (2) Standoff distance; (3) Parallactic distance; (4) Terminal wind speed; (5) Specific intensity}
\end{deluxetable*}

%The discovery of two distorted interstellar bubbles in \citet{GullandSofia1979} led the authors to interpret these structures as a feature formed from wind-driven mass loss. The arc-shaped nebula illustrates the boundary where the stellar-wind pressure equals the ram pressure from the flowing interstellar medium. In this view, the mass-loss rate of the central star can be given as a function of several observables in Equation~\ref{eq:one}. Building on this approach, \citet{K18} show that $\dot{M}$

In \citet{K18}, the authors showed that Equation~\ref{eq:one} can be rewritten as:

\begin{equation}
\begin{split}
    &\dot{M}\left(\moperyear\right) =1.67\times10^{-28}\times\\
    &\frac{\left[R_0\left(\arcsecs\right)\right]^2D\left(\kpc\right)\left[V_a\left(\kms\right)\right]^2I_\nu\left(\Jysr\right)}{V_w\left(\kms\right)\ell\left(\arcsecs\right)j_\nu\left(\Jycmsrnuc\right)}\text{.}
\end{split}
  %  \dot{M}\left(\moperyear\right) = 1.67\times10^{-28}\times\frac{\left[R_0\left(\arcsecs\right)\right]^2D\left(\kpc\right)\left[V_a\left(\kms\right)\right]^2I_\nu\left(\Jysr\right)}{V_w\left(\kms\right)\ell\left(\arcsecs\right)j_\nu\left(\Jycmsrnuc\right)}\text{.}
    \label{eq:two}
\end{equation}

%Trace space velocities forward from K22, different rotation curve. gaia correction

%XX layout differences from previous work EDR3, 

%Systemtatics with proper motioins

% WHat the choices are, whts new and changed.

%Heres the improvements and what we do

%Discussion, what difference would it have made if we had done different dust emissicity.
% fractional arcsec \farcs{1}{5}

\noindent where $R_0$ is the standoff distance between the star and the apex of the nebula, $D$ is the distance to the bowshock star, $V_a$ is the velocity of the star with respect to its surroundings, $I_\nu$ is the specific intensity of the emitting dust in the bowshock nebula, $V_w$ is the terminal velocity of the stellar wind, $\ell$ is the chord length across the bowshock arc, and $j_\nu$ is the dust emissivity per nucleon. The expression is linear for the quantities $D$, $I_\nu$, $V_w$, $\ell$, and $j_\nu$, while $R_0$ and $V_a$ take a squared dependence.

\begin{figure*}[htb!]
        \plotone{figures/BS692.eps}
        \caption{Three color image of \citep[object 692$_\star$ from][]{K16} with red/green/blue representing 160 and 70~$\um$ \textit{HSO} and 24 $\um$ \textit{SST} data respectively. The X marks the location of the driving star and the vectors depict the morphological parameters $R_0$ and $\ell$.}
        \label{fig:bowshock}
\end{figure*}
%XXzoom in, bold face fonts
%emphasie geen more
%X marks location of driving OB stars
%%bigger, bolder X
%XXBS885 in 160,70,24

%Define shortcut for K16, K18, K19

Figure~\ref{fig:bowshock} displays a three-color representation of the bowshock nebula surrounding G353.4162+00.4482 \citep[candidate 692$_\star$ from][]{K16}. Red and green depict archival \textit{HSO} 160 and 70~$\um$ images and blue represents \textit{SST} 24~$\um$ image. The bowshock is most evident at 24~$\um$ and is visible at 70~$\um$ but not at 160~$\um$. The bowshock is the dominant feature at 24~$\um$, but at 70~$\um$, both background and foreground nebulosity are visible. A white X marks the location of the driving OB star, which is not directly visible in the images. The yellow vectors illustrate the morphological parameters $R_0$ and $\ell$. To obtain $R_0$, we adopt the standoff distances measured by the citizen science project described in \citet{Whisnant2025}. They found overall good agreement between their crowd-sourced measurements for $R_0$ compared to single-measurement previous values. For the subset of stellar bowshock nebulae with ``small'' standoff distances ($R_0\lesssim10''$) as measured in K16, \citet{Whisnant2025} report their updated measurements of $R_0$ were systematically larger by $\sim$1\farcs5. We judge that the multiple measurements for $R_0$ obtained in \citet{Whisnant2025} are superior to the subjective measurements made by a single scientist in K16. XXthe nebulae are less well defined at 70. The 24 and 70 nebulae are coincident. We measure the chord length $\ell$ as the length across the arc .utilize archival \textit{SST} and \textit{HSO} survey data to measure the chord length $\ell$ by measuring .
%XX what Kobulnickt and Chick paper did.
%Slightly different velocities than K22, japanese author. 
%Gaia kinematic data and correcting solar motion.
% Distance and proper motion and solar motion wrt 
% Radial velocity.
% How well do space velocities agree?
% Tabulate parameters
% Galpy package that will compute velocities
% Venn diagram of O, B, runaway, BS stars.

Another required parameter is the velocity of the star relative to the surrounding ISM, $V_a$. K19 and K22 estimated this quantity from Gaia DR2 and EDR3 proper motion and parallax data, respectively. However, proper motions must be corrected for solar motion relative to the Local Stand of Rest and the adoption of a Galactic circular velocity as a function of Galactocentric distance (i.e., a galactic rotation curve). K22 performed this analysis on bowshock stars with available proper motions and parallaxes as well as on a control sample of non-bowshock GOSC stars. \citet{Carretero-Castrillo23} (hereafter shortened to C23) performed a similar runaway analysis of Galactic O stars using Gaia DR3 proper-motion data with some differences in their methodology compared to K22. C23 applied the zero-point correction to the Gaia parallaxes \citep[described in][]{Lindegren2021} while K22 did not. C23 also used a different rotation curve and solar motion with respect to the Local Standard of Rest (LSR) to compute the peculiar 2D space velocity.

\begin{figure}[htb!]
        \plotone{figures/GOSC_comps.pdf}
        %\plotone{figures/GOSC_comps_gal.pdf}
        \caption{The ratio of the \citet{Carretero-Castrillo23} (C23) to the \citet{K22} (K22) space velocities for the 23 GOSC stars studied in both works as a function of K22 peculiar 2D space velocity. The dashed line and the shaded region correspond to the median and variance in the comparison ratio.}
        \label{fig:GOSC_comparison}
\end{figure}

%XX Ratio, calculate dispersion.
% Plot ratio, them/us vs galactic longitude
% local s adoption of galcactic rotation curve, solar motion wrt lsr. velocities fall in this range and uncertainties are XX%

%XXPut second plot in thesis

Figure~\ref{fig:GOSC_comparison} plots the ratio of the C23 to the K22 peculiar 2D space velocities for the overlapping subsample of 23 GOSC stars analyzed in both works as a function of the K22 values. The horizontal dashed black line shows the median ratio of 0.92. The grey band encompasses the RMS of 0.12. Overall, there is a strong correlation between the two independent determinations of velocity. Because of a difference in methodology, C23 reported slightly higher uncertainties than the K22 measurements. XXAverage uncertainty of this vs this. The uncertainties we plot in Figure~\ref{fig:GOSC_comparison} represent the K22 and C23 uncertainties added in quadrature. Low-velocity stars on the left side of the plot have a typical uncertainty of 5~$\kms$ which amounts to 20\%, while the fastest stars at 90~$\kms$ have the same nominal uncertainty of 5~$\kms$ which represents only 7\%. Furthermore, the differences between K22 and C23 do not correlate with galactic longitude as might be expected if systematic differences in the galactic rotation curve were responsible. The difference between the K22 and C23 values could arise from the choice of mean solar motion with respect to the LSR and the choice of application zero-point offset correction to the Gaia measurements.

%XX Typical unceertaintiy which amount to % uncertainty. The typical uncertintiye sreported by both uhtors re 5--10 which amounts to XX for the slowest stars, but only 6% ofor the fastest stars at 90 kms. slow strs hve higher uncertinties.

% Additional improvement to K18/K19. uniformly 10% errro. We see that isnt the case adn we take a more careful star by star analysis of the uncertainties.

% While there is a 10 % offsett, the RMS about thge oen-to one is 15 % if we were to consider systematic errors in the computation, its possible our values are too high by 10%, squared, save for end. sars local frame. they range tabulate space velocities. Range from 15 kms to 90 kms. Heres where we tabulate. potentially as large as XX at the lower velocity end. Furthermore there may be systematic undercinty that result from ones choice of galactic rotition curve or men solr motion wrt the lsr. CC23 did with different, lower thn 9%. we tke this s  mesure of systemtic uncertinties. rotion curve, solr motio, nd possible sero point offset. possible issues with systemtics we my hve to reutrn to lter in the discussion.

%XX HSO data.

%XX Look into Mokiem, who cited Mokiem and do better

% XX Hawcroft

In Equation~\ref{eq:two}, we take $V_W$ to signify the terminal-wind speed of the stellar outflows. The terminal-wind speed is easily measurable from the P-Cygni profiles of metal-resonance lines in the UV, which every OB star exhibits. \citet{Mokiem2007} compiled wind parameters obtained from UV-based spectroscopic analysis for 49 Galactic O- and early B-type stars with effective temperatures ranging from 25--47~kK (Table A.1 in their Appendix). They reported terminal-wind speeds ranging from 1500~$\kms$ for the coolest stars to 3200~$\kms$ for the hottest stars. Since UV spectra do not exist for our sample of bowshock stars\footnote{Exceptions $\zeta$ Oph (BS013$_\star$), HD 195592 (BS343$_\star$), HD 199021 (BS345$_\star$), HD 41161 (BS$374_\star$), V* AE Aur (BS375$_\star$), HD 48099 (BS375$_\star$), $\upsilon$ Ori (BS378$_\star$), HD 54662 (BS381$_\star$), V* GP Vul (BS386$_\star$), HD 153426 (BS662$_\star$), V* V1012 Sco (BS667$_\star$), and $\kappa$ Cas (BS794$_\star$).} K18/K19 used the results of \citet{Mokiem2007} to estimate the terminal-wind speed for their sample, with $\teff$ approximated from rough spectral types in the literature. In this work, we adopt the $v_\infty$--$\teff$ calibration  of \citet{Hawcroft2024}, which used 66 Galactic OB stars spanning 15 kK -- 45 kK from the UV spectroscopic study of \citet{HowarthandPrinja1989} with updated stellar parameters provided by \citet{Holgado2020}. The \citet{Hawcroft2024} relation shows little-to-no dependence on luminosity class---no $v_\infty$ dependence on $\logg$. Their relation shows a scatter with an RMS of 277~$\kms$. We add this RMS in quadrature to the error produced by the uncertainty in temperature measured in \citet{Patten2025}.

%XX Systematics logg??, different data points for different logg on v T plot.

%Look at southern starsXX, look at K19/K18

%XX T range for Hawcroft

%XXTHere dont exist UV spectra for any BS star and so we adopt the Vwind Teff cal from MOkiem. Owing to the infeasibility of obtaining UV spectra for the bowshock sample, they approximated the spectral of each bowshock star from existing literature and interpolated over the tabulated \citet{Mokiem2007} values. From this method, K19 claimed to measure $V_W$ to within 20\%. K18/K19 used the results of Mokiem to assign v infty as a function of temperature.

%We use the fit of \citet{Hawcroft2024}, which is based on the much larger of 66 OB stars from \citet{HowarthandPrinja1989}. study with updated stellar parameters from. They show that it is well approximated by a linear relation between vwind and Teff with a dispersion of XX kms.

%Discussion In an update to \citet{Mokiem2007}, \citet{Hawcroft2024} studied the metallicity dependence on terminal wind-speeds using newly acquired UV spectra from the Hubble Space Telescope UV Legacy Library of Young Stars as Essential Standards (ULLYSES) program and existing measurements in the literature. In their study of Galactic stars, they draw 66 OB stars with saturated \ion{C}{4} $\lambda\lambda$1548--1551~\angstrom~profiles (i.e. well-defined $v_\infty$) from \citet{HowarthandPrinja1989}, with updated measurements of stellar parameters (e.g. $L_\star$, $\teff$, $\logg$, etc.) as measured in \citet{Holgado2020}. From these data, \citet{Hawcroft2024} demonstrated the empirical relation between $v_\infty$ and $\teff$ (Equation 5 in their study). In this work, we apply the \citet{Hawcroft2024} relation to obtain $V_W$ for our bowshock sample. In addition, we also report an uncertainty in the wind speed we calculate, based on error propagation from the RMS of the fit in \citet{Hawcroft2024} and the uncertainty is $\teff$ from \citet{Patten2025}.

%GIve reange for T

%\begin{figure}[htb!]
%       \plotone{figures/Vw_comp.pdf}
 %       %\plotone{figures/GOSC_comps_gal.pdf}
%        \caption{The ratio of the empirical stellar-wind speeds from the \citet{Hawcroft2024} to the terminal-wind speeds adopted in K19 plotted against the K19 values for the overlapping 24 stars studied in both works. The dashed line indicates the median ratio and the shaded regions correspond to the RMS.}
%        \label{fig:Vw_comparison}
%\end{figure}

% Maybe move to discussion

%Figure~\ref{fig:Vw_comparison} plots the ratio of this work's $V_W$ to the K19 wind speed as a function of the K19 values for the 24 stars in common with this work's and K19's sample. Each point displays the uncertainty in the ratio based on uncertainty in the wind-speed value from K19 and this work. The horizontal dashed line indicates the median ratio of the 24 stars and the shaded regions correspond to the RMS value of the ratio. Both estimations of stellar-wind speeds are in agreement with each other over the range of measured stellar-wind speeds in K19, considering either the random variation or the uncertainties in each speed value. However on average, this work's reported stellar-wind speeds are approximately 25\% greater than the K19 values, which could indicate a systematic reduction in this work's mass-loss rates by 25\% compared to K19.

For distance $D$ we adopt the inverse parallactic distance provided by Gaia DR3 to obtain $D$.

We measure the specific intensity at $I_\nu$ from archival \textit{HSO} 70 $\um$ UNIMAPB level 2.5 images from the Photodector Array Camera and Spectrometer (PACS) photometer in parallel mode (pixel size 3\farcs2). Most of the 24~$\um$ were obtained from the MIPSXX\citep{Molinari2010}. In cases where there is structure in the bowshock or confounding background emission, we found it necessary to smooth the images by 1--3 pixels to increase the signal-to-noise ratio. The peak surface brightness in 70~$\um$ coincides with the peak surface brightness in 24~$\um$XXIn most cases...however it some instances where the field has contaminating background and foreground emission the peak location of the 70 um is unclear. We assume the two peaks are coincident and use the peak in 24 emission to measure the peak in 70 um. 70 is dominated by larger dust grains which may be exterior to the shock fron where the smaller grains arte located. Using adjacent regions on either side of the peak along the line of $R_0$, we estimate the background flux. Fitting a linear baseline on either side of the peak. We subtract this estimate of the background from the peak brightness along $R_0$ to measure the background-subtracted peak flux. Location in the table of the 70 um peak and the uncertainty.

\begin{figure*}[htb!]
        \plottwo{figures/BS016.eps}{figures/bowshock_multiwavelength.pdf}
        \caption{Left: Three color image of \citep[object 016$_\star$ from][]{K16} with red/green/blue representing 160 and 70~$\um$ \textit{HSO} and 24~$\um$ \textit{SST} data respectively. Right: The brightness along $R_0$ in arcseconds for 24~$\um$ (blue) and 70~$\um$ (green).}
        \label{fig:bowshock_multi}
\end{figure*}

Figure~\ref{fig:bowshock_multi} displays on the left a three-color representation of the bowshock nebula surrounding candidate 016$_\star$ in K16 in the same color mapping as in Figure~\ref{fig:bowshock}. The right panel displays the surface brightness of the bowshock nebula along the $R_0$ vector with the left axis corresponding to the 24~$\um$ data and in units megaJanskys per steradian and the right axis corresponding to the 70~$\um$ data in units Janskys per square pixel. The 24~$\um$ peak brightness is 0.24~$\MJypersr$ and the 70~$\um$ peak brightness is 125~$\Jypersquarepix$ for this nebula. The peak of the nebula are slightly offset from each other by about 17\farcs8. The 70~$\mu$ data shows a lot of background emission from nebular features while the 24~$\um$ is relatively uncontaminated.

% Some cases unrelated background and foreground. We take the location of the 24 um peak to measure the

%XX Approach and difficulties. We HSO 70 maps and which version we used. Smoothing technique we used. Provide plot of 70 and 24 overlap. The smoothed data show that the 24 and 70 peaks overlap. To increase S/n we smooth by XX pixels and fit a gaussian pek to obtaint a robust measurement of I70, I 70 from K19 by fact of 4 stemming from pixel size. The smoothing and fitting the peak is more robust measurement of I-70 than the K/18/K19.

%XX Figures to show range and outlier.s Histograms, scatter plots. Talk about what we get. Scatter for l and R_0. log U vs R_0. Think of parameters that belong together. U and R_0. T vs R_0. common x axis R_0 and other params on y-axis. R_0, I_nu, ell, j_nu. interelations. U. spread in daya, correlations. j_nu dependes. error analysis. some will cancel out. more or less sensitive to r_0. v_a vs D.

% Table XX lists the fundamental params for each of the terms in euation. point toward column in table in concluding sentence python,

%XX systematics in discussion

%Lastly, we estimate the dust emissivity per nucleon $j_\nu$ from modeled emission spectra (see Section~\ref{subsec:j_nu} further elaboration).

Most of the parameters in Equation~\ref{eq:two} are readily observable from optical and infrared data and require few assumptions. The major exception to this is $j_\nu$, which must rely on an adopted set of theoretical properties for dust grains. We adopt the \citet{Draine2021} models to compute $j_\nu$. \citet{Draine2021} modeled the dust infrared emission as a function of different radiation field intensities $U$, spectral energy distribution of the stellar population heating the dust, and dust compositions. $U$ is defined as

%To account for different XXefficiencies in dust heating for different stellar populations, the authors parameterize their models by the dimensionless energy density parameter $U$ defined as:

%We estimate the dust emissivity per nucleon $j_{\nu}$ from modeled dust emission spectra. 

%\citet{DraineandLi2007} (shortened to DL07) modeled the emission spectra of interstellar dust heated by varying radiation fields and tabulated the emission per nucleon over a range of infrared wavelengths. The models are parameterized in terms of the PAH composition fraction $q_{\text{PAH}}$, as well as the minimum and maximum strength of the interstellar radiation field (ISRF) to which the dust is exposed and heated. DL07 quantify the strength of the ISRF with the dimensionless parameter $U$---the ratio of the modeled ISRF to the ISRF of the solar neighborhood estimated by \citet{MMP83} and given by the equation:

%\begin{equation}
%    U=\frac{u_*}{u^{\text{MMP83}}}\text{ ,}
%\end{equation}

%\noindent with $u^{\text{MMP83}}=2.17\times10^{-2}~\ergscmc$. DL07 only considered the ISRF in the solar neighborhood, which led some to consider the effects there are on dust emissivity when considering heating from different stellar radiation fields. \citet{HenneyandArthur2019} model the grain emissivity of dust heated by early-type stars. In their work, they found that their dust emissivity at $70~\um$ was significantly higher than the \citet{DraineandLi2007} values. They argued that since the SED of an OB star peaks in the UV, the radiation field from an OB star is much more efficient at heating dust grains compared to the local ISRF for the same $U$. Consequently, \citet{HenneyandArthur2019} scaled the radiation field parameter $U$ by a factor of 8 to rectify this difference.

\begin{equation}
    U = \gamma_*\frac{u_*}{u_{\text{mMMP}}}\text{ ,}
\end{equation}

\noindent where $\gamma_\star$ is a model-dependent factor and $u_{\text{mMMP}}$ is the modified mean interstellar radiation field (ISRF) used by \citet{Draine2021} ($u_{\text{mMMP83}}=3.1293\times10^{-2}~\ergscmc$), which in turn is based on the mean ISRF energy density  ($u_{\text{MMP83}}=2.17\times10^{-2}~\ergscmc$) calculated by \citet{MMP83}. We compute $u_*$---the energy density at the apex of the infrared nebula---from

\begin{equation}
    u_* = \frac{R_*^2\sigma\teff^4}{R_0^2c}\text{ ,}
\end{equation}

\noindent where $R_*$ is the radius of the star, $\teff$ is the effective temperature of the star, and $R_0$ is the standoff distance. \citet{Draine2021} calculated the dust emissivity for three different irradiation spectral energy distributions: young stellar populations with different ages, an updated ISRF, and bulge stars. \citet{Draine2021} used the BPASS \citep{BPASS, BPASS2} and BC03 \citep{BC03} models to provide the input spectral energy distributions for the young star populations. They considered several different dust compositions that included different PAH ionization distributions (high, standard, and low ionization) and particle size distributions (large, standard, and small particles). We adopt the \citet{Draine2021} emissivities calculated from the BPASS tracks at solar metallicity and age 10~Myr to best reflect the stars at the center of bowshock nebula. We also select the models with standard grain size and ionization distributions. We interpolate between models to obtain $j_\nu$ as a function of $U$. Our approach differs from the one adopted in K19 in that we now have available modeled $j_\nu$ as heated by young star populations and we do not require an ad hoc correction suggested by \citet{Henney2019}.

%XXThe dust emissivities are most streongly a function of U and not particularly sensitive to stellar age and dust grain compoisition.

\begin{figure}[htb!]
        \plotone{figures/compare_DLO7.pdf}
        \caption{\citet{DraineandLi2007} dust emissivity compared to \citet{Draine2021} dust emissivities at $70~\um$.}
        \label{fig:compare_DL07}
\end{figure}

%Updated label on figure to remove M31

We consider systematic effects from our choice of models by comparing the dust emissivities at 70~$\um$ for the available set of models. Figure~\ref{fig:compare_DL07} plots the dust emissivity at 70~$\um$ for several dust emission models as a function of radiant energy density divided by model $\gamma_\star$. This shows the effect of heating efficiency over the different stellar populations. The purple line with filled circles denotes the mMMP dust emissivities tabulated in \citet{DraineandLi2007}, the cyan curve with filled crosses represents dust emission when heated by very old bulge-star populations, the pink curve with upside down triangles displays \citet{Draine2021} ISRF dust emission, and the yellow track with triangles represent the BC03 10 Myr stellar population at solar metallicity. All emissivity curves are normalized to the BPASS models at 10 Myr. The largest deviations from the BPASS models occur for the very old bulge stars, with the bulge star emissivities rougly equaling 20\% the BPASS emissivities for small $U$, and the bulge star emissivities 40\% the BPASS emissivities on the high $U$ end. The next highest deviations from the BPASS models are the \citet{DraineandLi2007} and \citet{Draine2021} mMMP set of models, with their emissivities 30\% the BPASS emissivities for low $U$, and the ratio increasing to about 60\% for high $U$. In close agreement to the BPASS emissivities are the BC03 models, with deviations $\lesssim$1\% over all $U$.

\begin{figure}[htb!]
        \plotone{figures/compare_ages.pdf}
        \caption{Ratio of dust emissivity at 70 $\um$ for a given heating stellar population to $j_{70}$}
        \label{fig:compare_ages}
\end{figure}

We also consider differences that arise in our choice of model parameters. Figure~\ref{fig:compare_ages} plots the dust emissivity calculated at 70 $\um$ heated by single-age stellar BPASS models over the single-age stellar population ages 3, 10, 100 and 300 megayears. All tracks are normalized to the 10 Myr track. All emissivities agree to within $\sim$5\% over the range of $3\leq U\leq5$. On the low $U$ end, the 3 Myr track is still in good agreement with the 10 Myr model with differences of 3\%. Relatively larger deviations are exhibited for the 100 and 300 Myr models on the low $U$ end, with differences exceeding 12\%. Since the central stars to bowshock nebulae were shown to be almost exclusively to be OB stars in previous works \citep{Patten2025}, the 3 and 10 Myr comparisons are most pertinent to this study. Subsequent comparisons to the other free parameters---choices of grain-size distribution and ionization distrubtion---were shown to alter the dust emissivity to significantly smaller degrees.

%\begin{figure*}[htb!]
%        \plottwo{figures/stacked_stellar.pdf}{figures/stacked_morph.pdf}
%        \caption{Ratio of dust emissivity at 70 $\um$ for a given heating stellar population to $j_{70}$}
%        \label{fig:stacked_summary}
%\end{figure*}

%\begin{figure*}[htb!]
%        \plottwo{figures/T_j_nu.pdf}{figures/T_R_0.pdf}
%        \label{fig:correlations}
%\end{figure*}

%Most of the parameters \citet{K18, K19} showed the mass-loss rate depend on are readily observable from optical and infrared data and require little assumptions. The major exception to this is $j_\nu$, which must rely on simulated data and requires a set of assumptions on the properties of the interstellar dust.

%XX Maybe subsection for j_nu

%Figure~\ref{fig:compare_ages} directly compares the \citet{DraineandLi2007} modeled dust emissivity at 70 $\um$ with the updated dust-model emissivity from \citet{Draine2021}. For the \citet{Draine2021} values, we adopt the \citet{BC03} radiation field at solar metalicity and age of 10 Myr. When considering the radiation field from a young population of stars, we find the resultant dust emissivity at 70 $\um$ to be lower by a factor of 1.13. This is in direct contrast to the findings of \citet{HenneyandArthur2019} in which they suggested increasing the radiation field intensity $U$ to account for heating by an early-type star, effectively up-scaling the \citet{DraineandLi2007} values! One possible source for this discrepancy is?XXtalk about CLOUDY???. For our study, we adopt the \citet{Draine2021} values.

%\begin{figure}[htb!]
%        \plotone{figures/j_70.pdf}
%        \caption{Completeness of bowshock sample.}
%        \label{fig:completeness}
%\end{figure}

% Stellar age j_nu tracks from Draine+21

% 

==> sections/target_selection.tex <==

XXOur targets lie betwene this galactic latitude and this longitude range, and distances. THere are XX targets outliers latitude.

% Bowshock catalogs
We selected a subset of the 709 targets cataloged in \citet{K16} and 311 tabulated in \citet{J19}. We selected for bright targets observable from the northern hemisphere to do follow-up spectroscopic analysis. These criteria resulted in 104 bowshock candidate stars studied in the previous work \citet{Patten2025}, in which optical blue spectra revealed these stars to be almost entirely single and binary early-type stars. These constraints also provided the subset of stars studied in \citet{Whisnant2025}. Citizen science through the online Zooniverse platform collected bowshock morphological parameters and individualized uncertainties on each parameter.

%XX Started with K16 and J19 catalogs. Good blue spectra from P25. High quality Gaia data

% Better job than what we did before. Start with P25 objects. Worth expanding???

% Don't have HSO, BS or noise?? Be inclusive for now. Case by case. We assume all due to O supergiant. ds9, iraf imcounts? python average over section. 

% Could write methods section. Introduce basics of bowshock techniques. Dont have to derive them. Same dust emissivities. Give enough of an intro so someone doesnt have to go back. Following K19 we adopt...

%XX use K19??
%XX DR3, DR4, HSO 70 um images, independently measuing 70 um intensity, background subtraction??
